The ALMA REBELS Survey. Epoch of Reionization giants: properties of dusty galaxies at $z \approx 7$

We analyse FIR dust continuum measurements for 14 galaxies ($z\approx 7$) in the ALMA REBELS LP to derive their physical properties. Our model uses three input data: (a) the UV spectral slope, $\beta$, (b) the observed UV continuum flux at $1500$A, $F_{\rm UV}$, (c) the observed continuum flux at $\approx 158\mu$m, $F_{158}$, and considers Milky Way (MW) and SMC extinction curves, along with different dust geometries. We find that REBELS galaxies have (28-90.5)% of their star formation obscured; the total (UV+IR) star formation rates are in the range $31.5 < {\rm SFR}/ (M_\odot {\rm yr}^{-1}) < 129.5$. The sample-averaged dust mass and temperature are $(1.3\pm 1.1)\times 10^7 M_\odot$ and $52 \pm 11$ K, respectively. In some galaxies dust is abundant (REBELS-14, $M'_d \approx 3.4 \times 10^7 M_\odot$), or hot (REBELS-18, $T'_d \approx 67$ K). The dust distribution is compact ($<0.3$ kpc for 70% of the galaxies). The dust yield per supernova is $0.1 \le y_d/M_\odot \le 3.3$, with 70% of the galaxies requiring $y_d < 0.25 M_\odot$. Three galaxies (REBELS-12, 14, 39) require $y_d > 1 M_\odot$. With the SFR predicted by the model and a MW extinction curve, REBELS galaxies detected in [CII] nicely follow the local $L_{\rm CII}-$SFR relation, and are approximately located on the Kennicutt-Schmidt relation. The sample-averaged gas depletion time is of $0.11\, y_P^{-2}$ Gyr, where $y_P$ is the ratio of the gas-to-stellar distribution radius. For some systems a solution simultaneously matching the observed ($\beta, F_{\rm UV}, F_{158}$) values cannot be found. This occurs when the index $I_m = (F_{158}/F_{\rm UV})/(\beta-\beta_{\rm int})$, where $\beta_{\rm int}$ is the intrinsic UV slope, exceeds $I_m^*\approx 1120$ for a MW curve. For these objects we argue that the FIR and UV emitting regions are not co-spatial, questioning the use of the IRX-$\beta$ relation.

==> REBELS Interpretation/definitions.tex <==

%%%%% AUTHORS - PLACE YOUR OWN COMMANDS HERE %%%%%

% Please keep new commands to a minimum, and use \newcommand not \def to avoid
% overwriting existing commands. Example:
%\newcommand{\pcm}{\,cm$^{-2}$}	% per cm-squared

% quick alias
\def\be{\begin{equation}}
\def\ee{\end{equation}}
\newcommand\code[1]{\textsc{\MakeLowercase{#1}}}
\newcommand\quotesingle[1]{`{#1}'}
\newcommand\quotes[1]{``{#1}"}
\def\gsim{\lower.5ex\hbox{\gtsima}} 
\def\lsim{\lower.5ex\hbox{\ltsima}} 
\def\gtsima{$\; \buildrel > \over \sim \;$} 
\def\ltsima{$\; \buildrel < \over \sim \;$} \def\gsim{\lower.5ex\hbox{\gtsima}} 
\def\lsim{\lower.5ex\hbox{\ltsima}} 
\def\simgt{\lower.5ex\hbox{\gtsima}} 
\def\simlt{\lower.5ex\hbox{\ltsima}} 
\newcommand{\ped}[1]{_{\mathrm{#1}}}



% solar stuff units
\def\msun{{\rm M}_{\odot}}
\def\lsun{{\rm L}_{\odot}}
\def\dsun{{\cal D}_{\odot}}
\def\fsun{\xi_{\odot}}
\def\zsun{{\rm Z}_{\odot}}
\def\msunyr{\msun/{\rm yr}}
\def\gdens{\msun\,{\rm kpc}^{-2}}
\def\sfrdens{\msun\,{\rm yr}^{-1}\,{\rm kpc}^{-2}}

% units
\def\mum{\mu {\rm m}}
\newcommand{\angstrom}{\mbox{\normalfont\AA}}
\def\cc{\rm cm^{-3}}
\def\uflux{{\rm erg}\,{\rm s}^{-1} {\rm cm}^{-2} }

% quantities defs
\def\fdust{\xi_{d}}
\def\fesc{f_{\rm esc}\,}
\def\td{\tau_{sd}}
\def\Sg{$\Sigma_{g}$}
\def\S*{$\Sigma_{\rm SFR}$}
\def\Ssfr{\Sigma_{\rm SFR}}
\def\Sgas{\Sigma_{\rm g}}
\def\Sstar{\Sigma_{\rm *}}
\def\Sesc{\Sigma_{\rm esc}}
\def\Srad{\Sigma_{\rm rad}}
\def\FUV{F_{\rm 1500}}
\def\FIR{F_{\rm 158}}


% additional wrappers for quantities and units
\def\Dsolar{${\cal D}/\dsun$}
\def\Zsolar{$Z/\zsun$}
\def\DDsolar{\left( {{\cal D}\over \dsun} \right)}
\def\ZZsolar{\left( {Z \over \zsun} \right)}
\def\kms{{\rm km\,s}^{-1}\,}
\def\skms{$\sigma_{\rm kms}\,$}
\def\msunyr{{\rm M}_\odot {\rm yr}^{-1}}


% LINES
\def\Scii{$\Sigma_{\rm [CII]}$}
\def\Sciimax{$\Sigma_{\rm [CII]}^{\rm max}$}
\def\CII{\hbox{[C~$\scriptstyle\rm II $]~}}
\def\CIII{\hbox{C~$\scriptstyle\rm III $]~}}
\def\OII{\hbox{[O~$\scriptstyle\rm II $]~}}
\def\OIII{\hbox{[O~$\scriptstyle\rm III $]~}}
% IONS
\def\HH{\hbox{H$_2$}~} 
\def\HI{\hbox{H~$\scriptstyle\rm I\ $}} 
\def\HII{\hbox{H~$\scriptstyle\rm II\ $}} 
\def\CIion{\hbox{C~$\scriptstyle\rm I $~}}
\def\CIIion{\hbox{C~$\scriptstyle\rm II $~}}
\def\CIIIion{\hbox{C~$\scriptstyle\rm III $~}}
\def\CIVion{\hbox{C~$\scriptstyle\rm IV $~}}
% ion variables
\def\nhh{n_{\rm H2}}
\def\nhi{n_{\rm HI}}
\def\nhii{n_{\rm HII}}
\def\fhh{x_{\rm H2}}
\def\fhi{x_{\rm HI}}
\def\fhii{x_{\rm HII}}
% MIX
\def\fd{f^*_{\rm diss}} 
\def\ks{\kappa_{\rm s}}

% COLORS
\def\cyan{\color{cyan}}
\definecolor{apcolor}{HTML}{b3003b}
\definecolor{afcolor}{HTML}{800080}
\definecolor{lvcolor}{HTML}{DF7401}
\definecolor{mdcolor}{HTML}{01abdf} %mahsa and davide
\definecolor{cbcolor}{HTML}{ff0000}
\definecolor{sccolor}{HTML}{cc5500} %stefano
\definecolor{sgcolor}{HTML}{00cc7a}

